Diversity Empowers Intelligence: Integrating Expertise of Software Engineering Agents

Large language model (LLM) agents have shown great potential in solving real-world software engineering (SWE) problems. The most advanced open-source SWE agent can resolve over 27% of real GitHub issues in SWE-Bench Lite. However, these sophisticated agent frameworks exhibit varying strengths, excelling in certain tasks while underperforming in others. To fully harness the diversity of these agents, we propose DEI (Diversity Empowered Intelligence), a framework that leverages their unique expertise. DEI functions as a meta-module atop existing SWE agent frameworks, managing agent collectives for enhanced problem-solving. Experimental results show that a DEI-guided committee of agents is able to surpass the best individual agent's performance by a large margin. For instance, a group of open-source SWE agents, with a maximum individual resolve rate of 27.3% on SWE-Bench Lite, can achieve a 34.3% resolve rate with DEI, making a 25% improvement and beating most closed-source solutions. Our best-performing group excels with a 55% resolve rate, securing the highest ranking on SWE-Bench Lite. Our findings contribute to the growing body of research on collaborative AI systems and their potential to solve complex software engineering challenges.

==> misc.tex <==

\subsubsection{Problem Formulation}

We formulate the SWE agent problem under the \textit{contextual Markov decision process} (CMDP) framework, represented by the tuple \( \mathcal{M} = (\mathcal{S}, \mathcal{C}, \mathcal{A}, \mathcal{R}, \mathcal{P}, p_0, \rho) \). The components are defined as follows:

\begin{itemize}
    \item \( \mathcal{S} \): State space, encompassing all possible states the agent could encounter, such as the current status of a file.
    \item \( \mathcal{C} \): Context space, including relevant repository information and issue descriptions.
    \item \( \mathcal{A} \): Action space, representing all potential actions or tools the SWE agent can utilize, such as \texttt{search} or \texttt{editing}.
    \item \( \mathcal{R} : \mathcal{S} \times \mathcal{A} \times \mathcal{C} \to \mathbb{R} \): Context-dependent reward function, providing scores for the actions taken by the agent.
    \item \( \mathcal{P} : \mathcal{S} \times \mathcal{A} \times \mathcal{C} \to \Delta(\mathcal{S}) \): Context-dependent transition function, defining how the state of the repository or information changes following a specific action.
    \item \( p_0 : \mathcal{C} \to \Delta(\mathcal{S}) \): Context-dependent initial state distribution.
    \item \( \rho \in \Delta(\mathcal{C}) \): Context distribution.
\end{itemize}

We formulate the SWE agent problem under the \textit{contextual Markov decision process} framework, which can be represented by a tuple \( \gM = (\gS, \gC, \gA, \gR, \gP, p_0, \rho) \). Here, \( \gS \) denotes the state space, which is a collection of all the possible the current agent could at, for instance, the current file status. \( \gC \) the context space, for example, the relevant repository information and issue descriptions. \( \gA \) the action space, i.e., all the possible actions or tools the SWE agent can use, for instance, \texttt{search} or \texttt{editing}. \( \gR : \gS \times \gA \times \gC \to \mathbb{R} \) is the context-dependent reward function, which provides scores for the actions taken by the agent. \( \gP : \gS \times \gA \times \gC \to \Delta(\gS) \) is the context-dependent transition function, i.e., how the repository or the information will change by applying a certain action. \( p_0 : \gC \to \Delta(\gS) \) is the context-dependent initial state distribution, \( \rho \in \Delta(\gC) \) the context distribution.

Given the initial context \( c \sim \rho \) and initial state \( s_0 \sim p_0(\cdot \mid c) \), at each time step \( t \), an agent follows a policy \( \pi : \gS \times \gA \times \gC \to \Delta(\gA) \) to select an action \( a_t \sim \pi(s_t, c) \) and receives a reward \( R(s_t, a_t, c) \). The action is then applied to the environment The environment then transitions to the next state \( s_{t+1} \sim P(\cdot \mid s_t, a_t, c) \).  and the agent receives a new state observation. As the iteration continues to time $T$, we are able to obtain a sampled trajectory \( \tau := \{s_t, a_t, r_t\}_{t=0}^{T} \). The goal for the agent is to maximize the cumulative reward along the trajectory, which can be described as a value function as follows.

\begin{equation}
    \max_{\pi} V^{\pi}(\rho) = \max_{\pi} \mathbb{E}_{\tau} \left[ \sum_{t=0}^{\infty} R(s_t, a_t, c) \mid c \sim \rho; \pi \right]
\end{equation}




